Human 3D keypoints via spatial uncertainty modeling

We introduce a technique for 3D human keypoint estimation that directly models the notion of spatial uncertainty of a keypoint. Our technique employs a principled approach to modelling spatial uncertainty inspired from techniques in robust statistics. Furthermore, our pipeline requires no 3D ground truth labels, relying instead on (possibly noisy) 2D image-level keypoints. Our method achieves near state-of-the-art performance on Human3.6m while being efficient to evaluate and straightforward to

==> fig/prior.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=.8\linewidth]{fig/2d_proj.png}
\caption{
Our model predicts a 3D Gaussian for each keypoint parameterized by $\mu, \Sigma$.
To supervise this prediction using 2D annotations, we differentiably project the 3D distribution onto each of the $C$ camera planes using para-perspective projection, yielding $C$ Gaussians with parameters $\{(\mu_c, \Sigma_c)\}$.
We then maximize the likelihood of the annotated keypoints in each image under the projected Gaussians.
\TODO{move images beside above the cameras, this image needs to be much smaller (half its current height)}
\TODO{update notation}
}
\label{fig:prior}
\end{figure}
